Software Model Evolution with Large Language Models: Experiments on Simulated, Public, and Industrial Datasets

Modeling structure and behavior of software systems plays a crucial role in the industrial practice of software engineering. As with other software engineering artifacts, software models are subject to evolution. Supporting modelers in evolving software models with recommendations for model completions is still an open problem, though. In this paper, we explore the potential of large language models for this task. In particular, we propose an approach, RAMC, leveraging large language models, model histories, and retrieval-augmented generation for model completion. Through experiments on three datasets, including an industrial application, one public open-source community dataset, and one controlled collection of simulated model repositories, we evaluate the potential of large language models for model completion with RAMC. We found that large language models are indeed a promising technology for supporting software model evolution (62.30% semantically correct completions on real-world industrial data and up to 86.19% type-correct completions). The general inference capabilities of large language models are particularly useful when dealing with concepts for which there are few, noisy, or no examples at all.

==> Content/2_background_further.tex <==
\subsection{Automatic Inference of Edit Operations}
% overview of mt learning in general is given in "Model transformation by-example: a survey of the first wave." and "Multi-step learning and adaptive search for learning complex model transformations from examples."
%\changed{Various approaches have been proposed to (semi-)automatically learn model transformations in the field of model transformation by example (MTBE).
%there are approaches that derive operations from the meta-model \cite{Kehrer2016, mazanek2009generating}, others rely on an operation recorder \cite{Langer2009, Gray2011, Kappel2012} and mining techniques can be used to derive further complex operations \cite{Kogel2016} and some propose to learn the model transformations from a set of given examples \cite{Kehrer2017, Mokaddem2018}. Operation recording and learning operations from a set of given examples is usually referred to as model transformation by-example (MTBE). Since we are interested in learning \eo{s}, we focus here on endogenous (i.e., source and target meta-model are equal) model transformations.
%We furthermore performed an informal literature review to be able to better put our case study into perspective of existing challenges in the area of model evolution and \sple{}. During our literature review, we did not find any research that is tackling the problems with a \cao{} approach to \sple{} in a practical setting. Some of the difficulties and challenges are mentioned by the research community, but research about how to overcome the challenges without starting from scratch and with the given constraints in an industrial setting is rare. 
% \subsection{Model Transformation \mbox{by-Example}}
%Even though some of the available tools allow for a visual, declarative definition of model transformations it is usually still a time-consuming activity and demands for the knowledge of another language that is not directly linked to the language the modeller is using.
%For example, \textsc{Henshin} rules are based on the abstract syntax but tool users are more familiar with the concrete syntax of their models. 
% I think this should be kind of obvious but if sources are needed, "MTBE: A survey of the first wave" mentions some references. But in Thesis also give an introduction into concrete vs. abstract syntax. The edit operations as we understand them are more like (possibly hidden) concepts. As such they have to be compared to concrete syntax and also Kehrers effective MMs. I think, in the end, these are all ways for efficient handling of concept hiding. 
%Therefore approaches have been proposed to learn model transformations from examples, so called \textit{model transformation by-example} (MTBE). It's important to distinguish here between exogenous, i.e., model and transformed model conform to a different meta-model, and endogenous model transformations, i.e., the models conform to the same meta-model.
%TODO add "From Examples to Knowledge in Model-Driven Engineering: a Holistic and Pragmatic Approach" as an important consideration how to derive good examples for learning.
Since simple operations on the abstract syntax graph of a software model are very fine-grained and may lead to inconsistent models, and since structural model differences are too specific, there has been a long history of attempting to infer \emph{relevant} \eo{s} (and model transformations in general) from available information (e.g., the \mmodel{}, given examples, or a model history).

\begin{definition}[Automatic Inference of Edit Operations]
Given a \mmodel{} $\mathcal{TM}$ with models $\mathcal{M}$, \emph{automatic inference of edit operations} is a computable function 
$I\colon 2^{\mathcal{M}} \to 2^{\mathcal{E}}$ that, given a set of models (and their \mmodel{}) $\mathcal{M}' \subset \mathcal{M}$, computes a set of \eo{s} $\mathcal{E}' \subset \mathcal{E}$.
\end{definition}

There are \emph{supervised} and \emph{unsupervised} approaches to the inference of \eo{s}.
One branch of supervised approaches are demonstration approaches, were a tool user presents the transformation steps to an operation recorder \cite{Yu2011,Langer2009}. Typically, these approaches require some manual post-processing, for example, edit conditions have to be refined manually \cite{Langer2009}.
Another branch of supervised approaches include by-example approaches, with which the tool user specifies a set of examples (and sometimes also counter examples) and the tool automatically infers the model transformations \cite{Jalali2012, Kehrer2017}. These approaches have been motivated by the seminal work of Varró \cite{Varro2006}, who proposed by-example learning for exogenous model transformations.
Furthermore, heuristic approaches \cite{Mokaddem2018} applying search-based techniques to finding a set of refactorings have been proposed. 
% THIS HAS NOT BEEN DONE; BUT WOULD BE A VALID EXTENSION OF OUR WORK (AS ALREADY STARTED IN THE EXTENSION OF THE ASE PAPER)
% If a set of \eo{s} is given, these can also be used to derive edit scripts and perform set-based assoiciation rule mining.

Unsupervised approaches include generative approaches, deriving model transformations from the \mmodel{}, and mining approaches.
Generative approaches have been proposed in the area of model transformation testing \cite{Brottier06mmfuzz}. Also, more recently, generative fuzzing approaches based on language models have been proposed that try to generate models with similar properties to real-world models~\cite{Shrestha2021SLGPT}. \Eo{s} are only indirectly addressed within these generative approaches. It has been shown that a complete set of consistency preserving \eo{s} can also be derived from the \mmodel{} \cite{Kehrer2016, mazanek2009generating}. These operations capture static constraints that are already present in the \mmodel{} and are typically very simple operations.
More recent MTBE approaches also use neural networks to learn exogenous model transformations, for example, Burgueño et al.~\cite{Burgueno2019, Burgueno201922} investigate learning exogenous model transformations from examples using long-short-term memory neural networks. However, these approaches need concrete input-output model pairs and have not been evaluated for endogenous model transformations.

Recently, mining model transformations from the modelling history using graph mining approaches has been proposed~\cite{Tinnes2021}.
\todo[inline]{Furthermore, in model optimization, it has been proposed to apply meta-heuristics... Also comparison of meta-heuristic and RL has been done... I think this is not close enough to mention here.
RL based Model Transformation (for optimization): https://ieeexplore.ieee.org/document/9592463/
}
An advantage of mining approaches over by-example approaches is that they do not require to handcraft examples. A disadvantage is their computational complexity and that negative application conditions and multi-object patterns (e.g., creating a variable count of elements in a model transformation) can not inferred.  Anyway, a post-processing (e.g., using by-example approaches) is conceivable, and it this sense, by-example approaches and mining approaches are orthogonal.
%To give a concrete example for the difference between $\mathcal{E}$, a generator $S$, and \eeo{s}, consider the modelling language SysML, which is used in system engineering~\cite{SysML2019}. The set $\mathcal{E}$ would then include very fine-grained elementary \eo{s} from $S$, for example, adding a port to a component or adding a connector between two ports, but also very large \eo{s}, for example for setting up the entire system architecture of a manufacturing execution system. An \eeo{} could be given, for example, by ``adding an interface'', that is, adding source port, target port, and connector in one step. After a port has been added to a component, a \ceo{} could be the completion of adding a target port and connecting the ports via a connector.

% \begin{definition}
%     An \emph{\eo{}} is an (endogenous) model transformation \cite{Biermann2012} that transforms a valid model $m_1 \in \mathcal{M}$ into another valid model $m_2 \in \mathcal{M}$.
% \end{definition}

% The set $\mathcal{E}$ of all \eo{s} acts on $\mathcal{M}$ as an inverse monoid.
% Ignoring (non-)application conditions, an \eo{} can be defined by a left-hand side graph $L$ and a right-hand side graph $R$ and a matching $K$ between the preserved nodes in $L$ and $R$ (i.e., $L \supseteq K \subseteq R$). 
 
% We can define an equivalence relation on the set of \eo{s} by
% \begin{align*}
% \varepsilon_1 &\sim \varepsilon_2, \quad \text{if and only if}\, \\
% SCG_{\Delta\left(\mathcal{M}, \varepsilon_1(\mathcal{M})\right)} &= SCG_{\Delta\left(\mathcal{M}, \varepsilon_2(\mathcal{M})\right)}, 
% \end{align*}

% where by $SCG_{\Delta\left(\mathcal{M}, \varepsilon(\mathcal{M})\right)}$, we denote the set of all \scg{s} of model differences between all valid models and the corresponding models after the application of the \eo{} $\varepsilon_1$. In this sense, the locality relaxation becomes a kind of forget operator on the set of \eo{s} $\mathcal{E}$ where attribute and matching information is lost. 

% It is straightforward to see that this relation indeed defines an equivalence relation. We can therefore define the quotient set $\mathcal{E}/\sim$, which---by construction---is set isomorphic to the set of \scg{s} that can be derived from the application of an .

% \todo[inline]{\begin{theorem}
% Suppose the size of the connected components is constant and the 
% and the number of pattern occurrences per subgraph is independent of the pattern. 
% Then serializing graphs and sampling most probable edges is equivalent to transaction based frequent subgraph mining.
% \end{theorem}

% \begin{proof}
% Step 1: The probability of edge extensions is equivalent to the maximum independent set frequency measure, which obeys the downward closure property. \par
% Step 2: $f_{MIS} > f$, and therefore a probable edge extension will find frequent patterns. 
% \todo[inline]{WIP}
% \end{proof}}

==> Content/7_related_further.tex <==
\subsection{Further Related Work}

%TODO reuse Recommenders in MDE have been applied to the reuse of models and transformations. Regarding model reuse, SimVMA [132] recommends Simulink mod- els similar to the one that is being developed, and which the designer can import or clone for their reuse; REBUILDER [42] finds UML diagrams similar to a given query, and supports their full or partial compo- sition into the given design; Paydar et al. [100,101] propose a reuse technique whereby the designer provides an input UML use case diagram, the most similar use cases are retrieved from a model repository, and then the activity diagrams associated to these use cases are semi- automatically adapted to (i.e. reused in) the new usage context; Koschmider et al. [50,51,71] propose both a rec- ommender of process model fragments, and an explicit search facility to retrieve complete process models or fragments and insert them in the current modelling con- text, adapting them if needed; and Hermes [34–36] can incorporate model search strategies to find model ele- ments suitable for reuse. Being generic, Hermes can also be applied to meta-models.

%^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%We have already given an overview of the literature on inference of \eo{s} and model completion in \secref{sec:background}. 
%In this section, we give an overview of research related to our work, that is, inference of \eeo{s} and software model completion.

\todo[inline]{Model Repair}

%Model repair 

%\cite{neubauer2017automated} In particular, IntellEdit [93] ranks quick fix solutions to model inconsistency problems according to the least-change principle; 

%PARMOREL [11,53] determines the model repair actions based on the user preferences and on the experience gained from repairing under different personalisation settings
%he diagram predicate framework (DPF) [108] and the approach by Nassar et al. [91] implement repairs as transformation rules; DiaGen [82] represents models as hypergraphs and uses hypergraph patches to produce recommendations for repairing models


% From the Literatrue Study:
%TODO even more on repair necessary ?
%Refacola [130] uses constraint-based rules; BPMoQualAssess [60] pro- vides guidelines to improve the actual value of quality metrics for business process models; B-repair [24] is spe- cific to the B formal specification language and ranks the suggested repairs based on their estimated quality; Revision [98] tracks model inconsistencies to the edit- ing action originating them in the model history and fixes this action to obtain a consistent model; MDSafe- Cer [87] detects missing information for supporting key evidence in process-based argumentations, and recom- mends how to resolve such deviations; ASIMOV [38] assists in the co-evolution of models and meta-models by proposing model co-evolution actions that a meta- modeller must have defined previouslyand Anguel et al. [8] also tackle the co-evolution problem, but they automatically fix resolvable changes and recommend co- evolution actions to deal with non-resolvable changes. There are also some model repair approaches that do not tackle model conformance, but they target other kinds of model-related problemsIn particular, Mani et al. [79] compute repairs for input test models that make a code generator produce an incorrect output; in addi- tion to complete, the suggestions for fixing behavioural tests in SMART [47] can also be classified as repairs; the Business Application Modeller (BAM) [137] permits specifying temporal rules for process models and, for some types of rules, it recommends how to fix their vio- lations; and AMOR [21] is a model repository for model versioning that includes a recommender of possible res- olutions for model conflicts.With respect to meta-model repair, two of the works tar- get OCL integrity constraints [12,28]. Batot et al. [12] tackle the co-evolution of OCL constraints upon meta- model changes. Their approach recommends a ranked list of OCL modifications that are correctly typed by the new meta-model version and minimise the num- ber of changes and information loss. Clarisó et al. [28] repair OCL constraints which are too restrictive or too lax. Their method suggests weaker or stronger candi- date versions of the problematic constraint, and the user can select one of them
% From Manuels ReVision ICSE 2018 Paper:
%Most approaches to model repair [4] aim at a fully automated repair process. One common approach is to employ a (heuristic) search strategy, which often leads to a huge number of repair alter- natives and to repair proposals which are hardly comprehensible for developers. For instance, the model repair tools Echo [3], Badger [7] and EMF Model Repair [6] fall into this category.
%The only available recommender tool known to us is the Model/analyzer [8]. It handles one single consistency violation at a time and first determines the model elements affected by an in- consistency. For each element, a so-called abstract repair action is generated which gives a rough hint of how to modify this element in order to improve consistency. An inconsistency is resolved by choosing and instantiating a subset of the set of generated abstract repair actions. However, the number of proposals is still large, and the user has no guidance for assessing whether the effect of the proposed repairs is appropriate.
%Model Repair

A slightly different but similar research area focuses on model repair \cite{neubauer2017automated, nassar2017rule , mazanek2009generating }. 
Stephan proposes an assistant that suggest both similar complete model solutions and repair suggestions using clone detection in Simulink \cite{stephan2019towards}. \textsc{ReVision}~\cite{ohrndorf2021history} uses so-called consistency-preserving edit operations to detected the origin of inconsistencies and then uses the pre-defined \eo{s} to recommend repair operations. 
Other methods emphasize a fully automated repair, often utilizing a heuristic search strategy \cite{macedo2013model, pinna2015resolving}. 



\todo[inline]{Knowledge Graph Completion}
https://arxiv.org/pdf/2208.11652.pdf 

\todo[inline]{Molecular Graph Generation}
In cheminformatics and bioinformatics, language models have been investigated for molecular generation, that is, to the generation of (undirected) graphs~\cite{zhumagambetov2021transmol, bagal2021molgpt}. 
%Motif Generation via LM in Bio-/Chemical Datasets: https://project-archive.inf.ed.ac.uk/ug4/20212351/ug4_proj.pdf

\todo[inline]{Temporal Graph Forcasting}
GNNs for model completion 
https://arxiv.org/pdf/2207.00255.pdf
https://arxiv.org/pdf/2302.01018.pdf
http://proceedings.mlr.press/v139/meirom21a/meirom21a.pdf
%already in this paper? or for later on, idea for future work?

%Prompting on graphs: https://arxiv.org/pdf/2302.08043.pdf

%Learning functional properties of proteins with language models: https://www.nature.com/articles/s42256-022-00457-9.pdf 

%Graph-to-text generation: https://arxiv.org/pdf/2007.08426
%Neural language modeling for contextualized temporal graph generation: https://arxiv.org/pdf/2010.10077


%Search String (to be refined):
%("pretraining" | "pre-training" | "transfer learning" | "transformer" | "deep learning") ("model completion" | "model transformation" | "edit operation") ( "uml models" | "eclipse modeling framework" |  "Simulink" | "SysML" | "IEC 61131-3")
%First 11 pages

%(~"language models" OR GPT-3) AND ("motive" OR "graph pattern" OR "graph motif" OR "motif" OR "subgraph")

%Datasets:
%https://link.springer.com/content/pdf/10.1007/s10270-021-00883-0.pdf


%%%%%%%%%%%% PATTERN MINING %%%%%%%%%%%%%%%%%%%
%There are also approaches to mine change patterns in source code. For example, \cite{Dagit2013} propose an approach based on the abstract syntax tree, and \cite{nguyen2019} mine patterns based on a so called fine-grained program dependence graph. \inExtension{\cite{janke2020} derive \emph{fine-grained edit scripts} from abstract syntax tree differences and transform them to a graph representation for graph mining.}{}{} %propose an algorithm to identify source code change patterns by grouping changes in the abstract syntax tree (AST) and generalizing these groups by performing some anti-unification.  %The main difference is that Dagit et al. work on trees whereas \textsc{Ockham} works on a kind of abstract syntax graphs which already include domain knowledge given by the meta-model. 
%A more recent code change pattern mining algorithm is given by Nguyen et al. \cite{nguyen2019} which does not operate on the AST but on a so called fine-grained program dependence graph. They don't use generic (frequent) subgraph miners but propose their own approximation algorithm which utilizes knowledge about the change patterns and a clone detection technique for clustering. 
%There is also some work that focuses on mining design patterns from source code~\citep{Oruc2016, balanyi2003mining, ferenc2005design, dong2009review}.
%%%%Code - Differences%%%%
%The idea behind these approaches --- learning (change) patterns from a version history --- is comparable to ours. In contrast to these approaches, \textsc{Ockham} works on a kind of abstract syntax graph, which already includes domain knowledge given by the meta-model. 
%This can also be understood as background knowledge we can provide to the pattern mining, that is, there is no need to work on higher levels of abstraction, as, for example in our case, the M0-level of the Meta-Object Facility \cite{omg2013mof}.
%Furthermore, we do not use a similarity metric to detect change groups or frequent changes but use an (exact) subgraph mining approach. In model-driven engineering, one often has some kind of identifiers for the model elements, which makes the differencing more reliable and removes the need for similarity-based differencing methods.
\todo[inline]{Source Code Completion}
Furthermore, it needs to be mentioned that for source code, the use of language models for code completion is outperforming other approaches and capable of generating code from natural language input~\cite{chen2021codex, ciniselli22}. Sobania et al.~\cite{Sobania2021GPvsGPT} compare large language model-based GitHub CoPilot to genetic programming based program synthesis. Wan et al.~\cite{wan22} study if abstract syntax tree representations can be retrieved from language models trained on code.

paper prem https://dl.acm.org/doi/abs/10.1145/3551349.3559555  or \cite{jesse2023large}

\todo[inline]{Model Generation (e.g., for mutation testing)}

"Pretraining for EMF/uml/Simulink"
Simulink GPT-2 Generation:
https://ranger.uta.edu/~csallner/papers/Shrestha21SLGPT.pdf

\todo[inline]{Program Synthesis}

An area of research related to inference of \eo{s} is automatic ``by-example'' program synthesis~\cite{gulwani2017program} such as Flash Meta~\cite{Oleksandr2015}. From the perspective of this kind of research, in the approach presented in this work, we try to learn a grammar. We haven't evaluated language models yet for identifying functional relationships between attributes in software models. Instead, our approach is able to detect patterns in the data and does not need any example pairs to derive these patterns. Therefore, the program synthesis approaches are more similar to the classical model transformation by-example approaches.
For the future, a combination of symbolic inductive programming approaches with neural approaches as the one presented here might be an interesting field of research.
%Stronger in our approach is that it works on complex structures not only sequential data.
%Therefore, it could be seen to be orthogonal. 
%A combination of neural approaches and symbolic and graph grammar learning probably should be a proper vision for the future.


\todo[inline]{Clone Detection}
% Elmar Jürgens work and others such as SimVMA

\todo[inline]{Knowledge Graph Extraction}

Some researchers investigate the extraction of knowledge graphs from language models~\cite{Swamy2021LM2KM, Garg2022CanLM}. Our idea of extracting \eeo{s} from a fine-tuned language model is similar in that we also try to extract ``learned knowledge'' from a language model. Anyway, our application domain is a different one.


==> Content/old_results.tex <==
\textbf{Experiment 1 (old):}
For 51.8\% of the simulated repositories, the generation procedure produced exclusively valid graphs, for 48.2\% it produced also only correct \scg{} (i.e., also correct with respect to the \mmodel{}). On average, $2.26$ invalid graphs are generated in the \generationPhase{}, with a minimum of $0$ and a maximum of $30$. A constraint in the given \edgel{} serialization is that a node with a given id has to appear always with the same label (i.e., the node labels are redundantly encoded in \edgel{}). The only type of violation against a valid \edgel{} encoding we have encountered in this experiment was that this correspondence of node id and node label has been violated. 
A manual inspection of the data for the model repositories with a large amount of invalid graphs ($>5$) reveals that these are the ``smaller'' datasets with mostly a high perturbation. For example, the repository with only 10 revisions, 11 applied \eo{s}, and a perturbation of 100\% is the one with the maximum of $30$ invalid graphs.

In \tblref{tbl:cor_faulty_graphs} we report the correlation coefficients (Spearman\footnote{We use Spearman correlation instead of Pearson correlation, since we can not assume that there are linear dependencies.}) between invalid graphs and invalid \scg{s}  and the base language model (BM), the number of training epochs, the perturbation probability (P), and the number of training tokens of the dataset (T). For the correlation with the base language model, we sort the base models according to their size (i.e., ada:~0, curie:~1, davinci:~2).

\begin{table}[bt]
\caption{Correlation (Spearman) between invalid graphs generation with other parameters. (**: $p < .001$, *:~$p < .01$)}
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{rSSSS}
  \toprule
 & {BM} & {Epochs} & {P} & {T}\\ 
  \midrule
  \#Invalid &  -0.08  & -0.10  &  0.35\,** & -0.33*  \\ 
  \#Invalid \mmodel{} & -0.22  & -0.05  & 0.31*  & -0.22   \\ 
  \#Invalid (+ davinci) & -0.28  & -0.11  & \text{--} & -0.56** \\ 
  \#Invalid \mmodel{} (+ davinci) & -0.24  & -0.13  & \text{--} & -0.56**    \\ 
   \bottomrule
\end{tabular}}
\label{tbl:cor_faulty_graphs}
\vspace{-1em}
\end{table}

We observe significant positive Spearman correlation between the number of invalid generated graph serializations and the perturbation parameter. Furthermore, there is a significant negative Spearman correlation between the number of invalid generated graph serializations and the number of tokens in the training set. 

\textbf{Experiment 2:}
At the token level, we find an average token accuracy of \averageTokenAccuracy{}, with a minimum of \minTokenAccuracy{}, and a maximum of \maxTokenAccuracy{} on our test data set.

Only \averageNumberCompletions{} completion candidates are generated, on average. For a large number of samples, only one \ceo{} candidate has been generated. In all of theses cases, the only candidate has also been the correct one.
On average, in \averageCorrectCompletion{\%} of the samples, the correct completion is among the candidates, with an average rank of \averageRankCompletion{} (w.r.t. the edge-scaled ranking).

In \tblref{tbl:cor_completion} we report on the Spearman correlation coefficients of the score of the completion candidates with the number of omitted edges (i.e., the ones that have to be computed), the total number of edges of the ground truth \scg{}, and the number of completions that have been generated.

\begin{table}[bt]
\caption{Correlation coefficients (Spearman) of the completion candidate score with the number of omitted edges in the sample, the number of total edges of the correct \scg{}, and the number of completion candidates that have been generated. (*: $p < .001$)}
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{rSSS}
  \toprule
 & {\#Omitted Edges} & {\#Total Edges} & {\#Completions}\\ 
  \midrule
  Score (best rank) & -0.69* & -0.38* &  -0.75*\\ 
  Score (best candidate) & -0.29* & -0.33* & -0.21*\\ 
   \bottomrule
\end{tabular}}
\label{tbl:cor_completion}
\end{table}

We see significant negative correlations between the score (of the best generated candidate and the best ranked candidate) and the number of edges that have to be completed, the number of edges from the full original \scg{}, and the number of completions candidates that have been generated. 

\textbf{Experiment 3:}
On average, out of the three applied \eo{s}, we could retrieve \averageCorrectAda{} for the \ada{} model, \averageCorrectCurie{} for the \curie{} model, and \averageCorrectDavinci{} for the \davinci{} model. The \davinci{} model has only been trained to the datasets that appeared to be difficult for \ada{} and \curie{} (i.e., perturbation probability of 100\%). %For these datasets, we were able to retrieve \averageCorrectAdaDifficult{} for \ada{} and \averageCorrectCurieDifficult{} for \curie{}, on average.

In \tblref{tbl:cor_retrieved}, we list the Spearman correlations of the correctly retrieved \eo{s} with the base model (BM), the number of training epochs, the perturbation probability (P), and the number of applied \eo{s} between two model revisions~(E).

\begin{table}[bt]
\vspace{-0.75em}
\caption{Correlations between the correctly retrieved \eo{s} and repository as well as language model parameters. (*: $p < .001$)}
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{rSSSS}
  \toprule
 & {BM} & {Epochs} & {P} & {E}\\ 
  \midrule
   \#Correct &  -0.33*  & -0.03  &  -0.80* & 0.10  \\ 
   \#Correct (+ davinci) & -0.22  & 0.08  & \text{--} & 0.28    \\ 
   \bottomrule
\end{tabular}}
\label{tbl:cor_retrieved}
\vspace{-1em}
\end{table}

The average generation cost for \ada{} was 0.45~Cent, for \curie{} 3.68 Cent, and for \davinci{} 51.84~Cent.

\textbf{Experiment 4:}
We list the MAP scores for the 4 different ranking metrics in \tblref{tbl:map_scores}.
Furthermore, we compare the average precisions obtained through the different ranking. We can observe a high significant ($p < .001$) Spearman correlations coefficients~$>0.65$ among all of them, the largest one between compression metric and node factorial scaled probability metric ($0.90$).




\begin{table}[b]
%\begin{minipage}[t]{.48\linewidth}
%\end{minipage}
%\begin{minipage}[t]{.48\linewidth}
\caption{MAP for the different ranking metrics. Grey background indicates the best MAP among all metrics.}
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lSSSS}
  \toprule
 & {Compression} & {Factorial} & {Probability} & {Edges-Scaled}\\ 
  \midrule
  MAP@3 & 0.32 & 0.20 & 0.13 & \cellcolor[gray]{0.9} 0.33 \\ 
  MAP@5 & \cellcolor[gray]{0.9}0.38 & 0.29 & 0.17 & 0.36 \\ 
  MAP@10 & \cellcolor[gray]{0.9}0.41 & 0.32 & 0.24 & 0.40 \\ 
  MAP@$\infty$ & \cellcolor[gray]{0.9}0.42 & 0.33 & 0.25 & 0.41 \\ 
   \bottomrule
\end{tabular}}
\label{tbl:map_scores}
%\end{minipage}
\vspace{-2em}
\end{table}

==> Content/related_full.tex <==
\section{Related Work}



\todo[inline]{
 Regarding research groups, I currently see the following ones
 1.) Li,Deng et al. in the area of process modelling. -> Pretty mature but these guys are focusing on process models and therefore are a little bit under the radar, tough from methods perspective they are top notch.
 2.) Kuschke, Mario Janke, Mäder -> Not sure if this research is still continued. Was reasonable but not top notch
 3.) Claudio Di Sipio, Juri Di Rocco, Davide Di Ruscio, and Phuong T Nguyen -> Not a lot behind. Very questionable graph contruction but they have a lot of fog in their papers that lets them appear more advanced... Looks like they apply the methods (which are trivial) to several use cases modify it only slightly and give it another name.
 4.) Heinemann, Adhikari,... not sure if this research is still continued. It was in the area of Simulink but reasonable, not top notch.
 5.) Elkamel -> Based on no "self-citations" I would assume that their efforts are discontinued.
 6.) Kögel, Langer, Raffael Groner,Tichy et al. reasonablke approach but  very likely discontinued because Kögel und Langer finished PhD longer ago.
 7.) SBSE stuff (i think discontinued). "too dumb" and therefore not interesting competitors.
8.) Martin Weyssow, Houari Sahraoui, and Eugene Syriani, Meriem Ben Chaaben, Lola Burgueño, Javier Cámara, Javier Troya, and Antonio Vallecillo, Jordi Cabot, and Sébastien Gérard -> do similar things to us therefore very relevant. Though they seem to focus on NLP. We could pass them by adding the GNN perspective. This group seems to be very distributed but large. Not sure but might be clever to look for a strategic partnership...}
In this section, we give an overview of existing work in the field of model completion and related fields. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Cluster 1 - Model Completion %%
Most relevant to our work is research in the area of software model completion. Various approaches have been proposed to address the challenges associated with model completion, ranging from rule-based approaches to data mining techniques and more sophisticated machine learning approaches. An overview of recommender systems in model-driven engineering is given by Almonte et al.~\cite{almonte22}.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Cluster 1.1 - Model Completion with rule-based approaches %%
Some of the previous work studies recommending model completions by utilizing knowledge bases such as pattern catalogs or knowledge graphs~\cite{agt2018domore,kuschke2017rapmod, kuschke2013recommending,maeder2021,li2013efficient,deng2016recommendation,minas2009}. For example, partial models can be completed by matching changes in catalogs of changes using pattern matching, graph matching, or other retrieval mechanisms, and then complete the model by applying the missing part of the identified change~\cite{kuschke2017rapmod, kuschke2013recommending,maeder2021,li2013efficient,deng2016recommendation,minas2009}. Other approaches utilize knowledge encoded in knowledge graphs and semantic web technologies to make recommendations during domain modeling~\cite{agt2018domore}. 
%RapMOD [72,73] offers auto-completion actions for (UML) graphical models, similarly to the vision paper [121]; Users' editing operations are analyzed and matched to a predefined but extensible catalog of common modeling activities for structural UML models. We found RapMOD to significantly reduce modeling effort. \cite{kuschke2017rapmod, kuschke2013recommending}  RapMOD [72] matches editing operations in UML structural diagrams to a catalogue of modelling activities and ranks the candidate activities by relevance RapMOD is implemented on top of the RETE-based Drools rule engine
Consequently, these research efforts are often domain-specific as they require the provision of domain-specific catalogs, such as for UML~\cite{kuschke2017rapmod,kuschke2013recommending,maeder2021} or business process modelling~\cite{deng2016recommendation, li2013efficient}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Cluster 1.2. - Model Completion with retrieval (AI) - Mostly Association Rule Mining
Another common approach is to use already existing model repositories and employ techniques such as frequency-based mining, association rule mining, information retrieval techniques, and clustering to suggest new items to be included in the model~\cite{adhikari2023simima,di2023memorec,di2023memorec, elkamel2016uml}. 
% Crossminer project - Similarity based retrieval
MemoRec~\cite{di2023memorec} and MORGAN~\cite{di2023morgan} present frameworks that use graph-based representation of models and model elements, and similarity-based information retrieval mechanism (e.g., graph kernels~\cite{vishwanathan2010graph}, cosine similarity of TF-IDF representations, or Jaccard index) to retrieve relevant items, such as classes and structural features, from a database of modelling projects. However, their graph-based representation is not directly related to the abstract syntax graph of the models and consequently may not capture the essential semantics and constraints of the modelling languages.
%Elkamel - Clustering
Elkamel et al.~\cite{elkamel2016uml} recommend UML classes, similar to the current modelling context, by utilizing a clustering approach on a collection of existing models. As a similarity measure, they use a combination of word-level similarities for name, attributes, and operations within a class.
%SimIMA: a virtual Simulink intelligent modeling assistant - Association Rule Mining
Adhikari et al.~\cite{adhikari2023simima} present a modeling assistant based on association rule mining and frequency based matching that suggests either new \textsc{Simulink} blocks to be added to the canvas or presents similar \textsc{Simulink} models based on a clone-detection~\cite{adhikari2023simima,stephan2019towards}.
% Association rule mining for simulink libraries
Heinemann~\cite{heinemann2012facilitating} proposes a collaborative filtering recommender system that uses association rule mining to suggest \textsc{Simulink} libraries for use.

%%%%%%%%%%%%%%%%%%%%%%%%%% 
%%%%%%%%%%%% Combination of 1.1 and 1.2
Repository mining and similarity-based item recommendation techniques are often combined. For example,
Deng et al.~\cite{deng2016recommendation, li2013efficient} combine pattern mining to built-up a pattern database from model history and then apply the rules from the database to the model completion for business process models.
K{\"o}gel et al.~\cite{kogel2016automatic,kogel2017recommender} identify rule applications in current user updates and find similar rule applications in the model's history. From these historic rule applications, they extract further, related rule applications and try to adapt them to the current user update context. The adapted related rule applications are then recommended to the user. In principle this can be seen as a combination of a association rule mining together with a catalog of higher-level change patterns/rules. %They assessed their approach using models from the Eclipse GMF project, focusing solely on meta models .
More generally, one could employ approaches to automatically compute minimal consistency-preserving rules~\cite{Kehrer2016} or pattern mining approaches~\cite{Tinnes2021,tinnes2023mining,langer2013posteriori} to derive a set of rules and then use them together with an association rule mining approach such as K{\"o}gel et al.~\cite{kogel2016automatic,kogel2017recommender}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Cluser 1.3 - Model Completion with SBSE approaches
Another strategy for model completion is to generate model completion candidates using search-based techniques~\cite{steimann2013}. These approaches use graph grammars or other techniques in combination with constraint solving to generate model completion candidates that comply with the given \mmodel{} and additional constraints. Without knowledge about any higher-level semantics, these approaches are therefore more comparable to the application of a catalog of minimal consistency-preserving \eo{s}~\cite{Kehrer2016}. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Cluster 1.4. - Model Completion with generative approaches (and other NLP approaches)

Regarding the application of natural language processing and language models, in particular, there has been some research activities in the model-driven engineering community:
Burgue{\~n}o et al.~\cite{burgueno2021nlp} propose an NLP-based architecture for the auto-completion of partial domain models. They do not employ language models in their approach and instead use other natural language processing approaches (i.e., word embedding similarity) to recommend words, which are then transformed into model elements in a post-processing.
Weyssow et al.~\cite{weyssow2022recommending} use a long-short-term memory neural network architecture to recommend \mmodel{} concepts but they do not generate entire model completions. 
Tsigkanos et al.~\cite{tsigkanos23} propose using language models to extract variables from user manuals for metamorphic testing.

While code completion and model completion are closely related, recent research has mainly concentrated on code completion, where large language models seem to be the state of the art \cite{chen2021codex, jesse2023large, ciniselli22m, Sobania2021GPvsGPT}. 


\todoa{ paper prem einbauen @christof? paper prem https://dl.acm.org/doi/abs/10.1145/3551349.3559555  or \cite{jesse2023large}}




Considering the close connection to code and model completion, it's essential for us to explore further how generative approaches, such as large language models, operate within the context of model completion. 
%Towards using Few-Shot Prompt Learning for Automating  Model  Completion
Most closely to the work presented here, is an approach by Chaaben et al.~\cite{chaaben2023towards}, which utilized the few-shot capabilities of large language models, specifically GPT-3, for model completion, eliminating the need for training or fine-tuning of models. In their study, they handpicked 30 domain models from the ModelSet dataset~\cite{lopez2022modelset, chaaben2023towards} and evaluated the effectiveness of the suggestions by simulating an incremental design process. 
The paper makes important contributions, but its reliance on static snapshots where elements are randomly removed could be enhanced to better reflect real-world complexities. In contrast to the handpicked few-shot examples, our approach takes a different avenue, leveraging model evolution from model repositories.
%To evaluate whether their approach leads to an effective suggestion of new classes, they began with 20\% of each model's elements as the a foundational diagram and simulated an incremental design process starting from this model \cite{chaaben2023towards}. Afterward, they performed two rounds of completion suggestions, after each round they validated the suggested results manually and added semantically correct elements for the next round
%\cite{chaaben2023towards}. They conducted similar experiments for Attributes suggestions and Association names suggestions. Their results show moderate recall and precision values. 
%They stated that their results varied based on domain specificity and the amount of natural language elements used %\cite{chaaben2023towards}.
%Towards using Few-Shot Prompt Learning for Automating Model Completion 
%On -> ums class diagrams and limited activity What few shot examples do they use: We create the prompt using some existing diagrams of unrelated domains, From these diagrams, we extract pairs of related classes, Sampling from model set: We consider 30 domain models, selected manually from the dataset ModelSet, What is removed: each model Mi, we take 20% of its elements as the already defined partial diagram M′i and we simulated an incremental design process starting from M′i. First, we performed a first round (R1) of completion suggestions, then we validated the suggested results manually adding to the model under- construction Mi’ those which were semantically equivalent to those elements in Mi To assess the effectiveness of our approach when suggesting new attributes within a class, we have selected randomly 212 classes from our dataset, have removed 75% of their attributes and have generated attribute completions for them. and the maximum number of tokens to 20 when generating suggestions for new classes (and their associations) and new attributes, and to 1 when suggesting association names. How is evaluation done: Precision, recall … on manually checked semantically correct items
%On the assessment of generative AI in modeling tasks: an experience report with ChatGPT and UML -> they do not really work on model completion, rather model creation Initial pilot study: We wrote prompts asking ChatGPT to create mod- els of different sizes, as well as to create the target models of some of the assignments that we use in our modeling lec- tures. The size of these models ranged from 10 to 40 classes and associations. Second experiment: Each author independently proposed ten UML models. small in size (three to six classes) so that ChatGPT could han- dle them without problems. one of them, the exercise consisted in asking ChatGPT to produce the corresponding UML model using one or more prompts. 
%Despite promising results for further investigation, the study lacks a real-world evaluation. \todoa{This needs to be more clear and less negative.  die evaluieren ja auf ModelSet und die sind schon real-world beinhalten aber keine real-world evolution da nur snapshots von repos aus denen random entfernt wird. außerdem ist fragwürdig, wie die den context erstellen. oder weißt du da mehr alisa? Wählen die die Beispiele für Few-Shot von hand aus oder irgendwie anders? Die Fragen gelten auch für Camara et al. Also da müssten wir uns nochmal von abheben, weil das ja ansonsten sehr ählich ist.}
%TODO On the assessment of generative AI in modeling tasks: an experience report with ChatGPT and UML https://link.springer.com/article/10.1007/s10270-023-01105-5
Cámara et al.~\cite{camara2023assessment} further extend on this research by conducting experiments to assess ChatGPT's capability in model generation. 
%In the first experiment, they tasked ChatGPT with creating models of varying sizes, from 10 to 40 classes and associations . 
%Base on the findings in experiment 1, in the second experiment eight smaller models, with the size of three to six classes were chosen from a pool of 40 UML models. Different strategies and series of prompts were used to evoke the desired models %\cite{camara2023assessment}. 
%Their findings include that ChatGPT usually generates syntactically correct models, both context and problem domain deeply influence the model outputs and that different prompts or strategies can yield varying results, and even when presented with identical prompts, ChatGPT can exhibit considerable variance in responses across different interactions \cite{camara2023assessment}. Further Cámara et al. highlight the limitation of ChatGPT being able to handel models of larger size, more than 10-12 classes already being problematic \cite{camara2023assessment}. 
%TODO model's semantics, aligning with the user's intent, is a weak point, with ChatGPT often suggesting irrelevant models. ChatGPT manages various modeling concepts some better than others

%Automatic Change Recommendation of Models and MetaModels Based on Change Histories https://ceur-ws.org/Vol-1706/paper3.pdf 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%% SUMMARY OF MODEL COMPLETION LITERATURE 2023 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%To summarize, there are five major tactics of software model completion in the literature: symbolic pattern matching, symbolic pattern matching of patterns derived from model histories, similarity-based model repository mining, search-based approaches, and generative approaches. Symbolic pattern matching requires the definition of the patterns and is therefore bound to specific models. Approaches that try to automatically derive the patterns from model repositories try to overcome this limitation but suffer from poor scalability and domain experts are required for curation of the pattern catalogs. Similarity-based mining is usually limited to recommendations of fine-grained changes such as recommending concepts for meta-models or recommending class attributes. Search-based approaches are usually limited to recommending syntactically correct completions and not capable of recommending higher-level completions. Also search-based approaches usually come up with large lists of recommendations and have no intrinsic means of further ranking these. Finally, generative approaches have only recently been proposed and seem to be promising. Further research is necessary though.

\todo[inline]{we can probably condense a nice table out of this comparison. Another property not mentioned in the current related work (because it would add another dimension and therefore complexity) is whether only partial models can be completed or all models can be completed etc.}


%^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^


\todoa{find right place for these 2 and make RW shorter}
A slightly different but similar research area focuses on model repair \cite{neubauer2017automated, iovino2020model, nassar2017rule , mazanek2009generating }. 
Stephan proposes an assistant that suggest both similar complete model solutions and repair suggestions using clone detection in Simulink \cite{stephan2019towards}. \textsc{ReVision}~\cite{ohrndorf2021history} uses so-called consistency-preserving edit operations to detected the origin of inconsistencies and then uses the pre-defined \eo{s} to recommend repair operations. 
Other methods emphasize a fully automated repair, often utilizing a heuristic search strategy \cite{macedo2013model, pinna2015resolving}. 

Some researchers investigate the extraction of knowledge graphs from language models~\cite{Swamy2021LM2KM, Garg2022CanLM}. Our idea of extracting \eeo{s} from a fine-tuned language model is similar in that we also try to extract ``learned knowledge'' from a language model. Anyway, our application domain is a different one.



==> Graphics/dataset_generation_flowchart.tex <==
\tikzstyle{block} = [rectangle, draw, fill=blue!20, 
text width=5em, text centered, rounded corners, minimum height=4em]
\tikzstyle{line} = [draw, -latex']

\tikzstyle{startstop} = [rectangle, rounded corners, 
minimum width=5cm, 
minimum height=1cm,
text centered, 
draw=black, 
fill=black!20]

\tikzstyle{io} = [trapezium, 
trapezium stretches=true, % A later addition
trapezium left angle=70, 
trapezium right angle=110, 
minimum width=5cm, 
minimum height=1cm, text centered, 
draw=black, fill=black!20]

\tikzstyle{process} = [rectangle, 
minimum width=5cm, 
minimum height=1cm, 
text centered, 
text width=3cm, 
draw=black, 
fill=black!30]

\tikzstyle{decision} = [diamond, 
minimum width=5cm, 
minimum height=0.75cm, 
text centered, 
draw=black, 
fill=black!30]
\tikzstyle{arrow} = [thick,->,>=stealth]


\resizebox{0.4\height}{!}{%
\begin{tikzpicture}[node distance=1.5cm, font=\large]

\matrix[matrix of nodes,column sep=3cm,row sep=1cm, ampersand replacement=\&]{
\node (in) [io] {Model Histories}; \&
\node (md) [process] {Model Differencing}; \\
\node (scg) [process] {Simple Change Graph Generation}; \&
\node (cc) [process] {Connected Component Computation}; \\
\node (filter) [process] {Filtering (too large)}; \&
\node (vdb) [process, yshift=0.15cm] {Vector Database Generation}; \\
\node (sample) [process, yshift=0.6cm] {Diversity Sampling Test Samples}; \&
\node (experiment) [decision, yshift=-0.8cm, align=center] {Sampling Strategy};\\
};

\node (few-shot-1) [process, below of=experiment, yshift=-0.95cm] {Similarity Sampling Few-Shot Samples};
\node (few-shot-2) [process, below of=sample, yshift=-2cm] {Random Sampling Few-Shot Samples};
\node (prompt-1) [process, below of=few-shot-1, yshift=-0.5cm] {Generate Prompts};
\node (prompt-2) [process, below of=few-shot-2, yshift=-0.5cm] {Generate Prompts};


\node (out-1) [io, below of=prompt-1] {Few-Shot Prompts Similarity-based};
\node (out-2) [io, below of=prompt-2] {Few-Shot Prompts Random};


\draw [arrow] (in) -- (md);
\draw [arrow] (md) |- ++(0,-1cm) -| (scg);

%\draw [arrow] (scg) |- (pro1);
\draw [arrow] (scg) -- (cc);
\draw [arrow] (cc) |- ++(0,-1cm) -| (filter);
\draw [arrow] (filter) -- (vdb);
\draw [arrow] (vdb) |- ++(0,-1cm) -| (sample);
\draw [arrow] (sample) -- (experiment.north);
\draw [arrow] (experiment) -- node[anchor=east] {Similarity} (few-shot-1.north);
\draw [arrow] (experiment.west) |- ++(0,0) -| node [above] {Random} (few-shot-2.north);
\draw [arrow] (few-shot-1) -- (prompt-1);
\draw [arrow] (few-shot-2) -- (prompt-2);
\draw [arrow] (prompt-1) -- (out-1);
\draw [arrow] (prompt-2) -- (out-2);


\end{tikzpicture}
}
